Defending Hardware-based Malware Detectors against Adversarial Attacks

In the era of Internet of Things (IoT), Malware has been proliferating exponentially over the past decade. Traditional anti-virus software are ineffective against modern complex Malware. In order to address this challenge, researchers have proposed Hardware-assisted Malware Detection (HMD) using Hardware Performance Counters (HPCs). The HPCs are used to train a set of Machine learning (ML) classifiers, which in turn, are used to distinguish benign programs from Malware. Recently, adversarial attacks have been designed by introducing perturbations in the HPC traces using an adversarial sample predictor to misclassify a program for specific HPCs. These attacks are designed with the basic assumption that the attacker is aware of the HPCs being used to detect Malware. Since modern processors consist of hundreds of HPCs, restricting to only a few of them for Malware detection aids the attacker. In this paper, we propose a Moving target defense (MTD) for this adversarial attack by designing multiple ML classifiers trained on different sets of HPCs. The MTD randomly selects a classifier; thus, confusing the attacker about the HPCs or the number of classifiers applied. We have developed an analytical model which proves that the probability of an attacker to guess the perfect HPC-classifier combination for MTD is extremely low (in the range of $10^{-1864}$ for a system with 20 HPCs). Our experimental results prove that the proposed defense is able to improve the classification accuracy of HPC traces that have been modified through an adversarial sample generator by up to 31.5%, for a near perfect (99.4%) restoration of the original accuracy.

==> classifier_old.tex <==
\begin{comment}
\subsection{Classifier Combination Analysis}
\label{sec:MTD:CCA}
When creating the moving target defense, multiple machine learning models are trained with different combinations of HPCs. As stated in Section~\ref{sec:background-HPCinML}, different manufacturers will have different numbers of HPCs in their processors. In addition, depending on the processor, only a certain number of HPCs can be read at a time using the {\it perf} command. This paper utilizes a {\it Raspberry PI 3 Model B} that supports 20 HPCs and the capability to read 4 HPCs per {\it perf} command. Using the combination formula, we can find the total possible number of HPC combinations that we can use to train machine learning models. After thorough mathematical analysis of the different possible combinations of HPCs in machine learning models, we have devised a generalized mathematical equation such that given the number of total HPCs available as well as the largest number of HPCs that a machine learning classifier can have, it will generate the number of total possible classifier combinations. First, constraints must be specified. In this situation, it is known that there will be some maximum number of HPCs available on the processor which we will call Y.
Therefore, the equation for the number of potential classifiers using some number {\it X} where X is $\leq$ Y, and X is the HPCs per classifier is calculated by $Y \choose X$. It is also assumed that we will have a constraint on the number of HPCs that the {\it perf} command can read which will be denoted as R. Lastly,it is also known that there will have to be some value Z which represents the maximum number of HPCs that each machine learning model can have. Z must be at least two because there has to be a minimum of 2 HPCs per machine learning model. If there is only one HPC in the classifier, an attacker can use the previously stated adversarial attack to deceive the model. By having at least two HPCs, even if the attacker targets one HPC, there is a good chance the other HPC will be unaffected. That is, 2 $\leq$ Z $\leq$ R. As a result, when Z is $\geq$ 2, we must sum the combinations starting from 2 up to Z. As an example, when Z is $\geq$ 2, the summation would be represented as:


\begin{equation} \label{equ5} No. \ of \ Total \ Classifiers  = {Y \choose 2} + ... + {Y \choose Z} \end{equation}


Using the generalized equation above, we can see that our generic equation must sum the total number of combinations given different Z values. That is, for an input of Z equals 2 and Y equals 20, we simply take combination of 20 and 2. However, when Z equals 4 and Y equals 20, we must take the summation of combination of 20 and 2, combination of 20 and 3, and combination of 20 and 4. Therefore, we can introduce sigma notation into our equation and start the count at 2 and iterate until we hit the value of Z. Equation~\ref{equ5} can now be represented as the following:

\begin{equation}
\label{equ6}
 Total \hspace{1mm} Classifiers\ (N) = \sum_{I=2}^{X}\hspace{1mm} {Y \choose I} : Z \hspace{1mm} \epsilon \hspace{1mm} [2,R]      
\end{equation}


In the equation above, {\it Y} is the number of total HPCs that are available in the processor while {\it Z} is the maximum number of HPCs that we can use per classifier. This equation utilizes variable X which is instantiated at 2 because as stated before, every machine learning classifier must have at least two HPCs in the moving target defense. We can see that the value of Z is contained between 2 and R inclusive. This will vary based on how many HPCs the {\it perf} command can gather.

Now that a formula for the number of potential machine learning classifiers that can be produced based off the number of available HPCs has been derived, one can now see how many different combinations of classifiers one can take. Let H be a value for the number of classifiers to be taken for the moving target defense from the total number of classifiers available which is N. H is constrained to 2 $\leq$ H $\leq$ N because the moving target defense must have at least 2 machine learning classifiers, but it can't be more than the total number of potential classifiers available. 


When H is 4, the combination of N and H, $N \choose H$ is calculated to find the number of combinations using only 4 classifiers. 
From equation~\ref{equ5}, one can build off this equation by replacing Y and Z for N. If the total number of combinations is desired, the summation of combinations starting from 2 up to N is calculated. The summation would be represented as:  

\begin{equation} \label{equ7} Total\ Combos = {N \choose 2} +...+ {N \choose N} \end{equation}


We can model this as a binomial expansion using:

\begin{multline}
\label{equ8}
  Total\ Combos = {N \choose 0} + {N \choose 1} +{N \choose 2} + {N \choose 3} +...+ \\  {N \choose N-1} + {N \choose N}
\end{multline}
 
Simplifying using the binomial theorem: 

\begin{equation}
\label{equ9}
  Total\ Combos = (1+1)^N - {N \choose 1} - {N \choose 0} \\
  = 2^N - N - 1
\end{equation}


Equation~\ref{equ9} above gives the total number of machine learning classifier combinations available given N which is the number of machine learning classifiers that can potentially be produced from X and H which are the number of HPCs per machine learning model and the number of total HPCs. 



Using the specified constraints to pick classifiers due to utilizing a {\it Raspberry PI 3 Model B}, the Y value is equal to 20 and the Z value will be a minimum of 2 with a maximum of 4. Z values will have a range of potential values because the machine learning models have to have at least two HPCs, but they can have a maximum determined by how many HPCs can be read per {\it perf} command. For a {\it Raspberry PI Model B}, utilizing equation~\ref{equ6} results in the total number of classifiers:


\begin{equation} \label{equ10} {20 \choose 2} + {20 \choose 3} + {20 \choose 4} = 6,175 \end{equation}



\begin{figure}
  \includegraphics[width=\linewidth]{Figures/hpcvsclass.png}
  \caption{Log Scaled Classifier Variation based on Total HPCs}
  \label{fig:hpcvsclass1}
\end{figure}


It is shown that using a {\it Raspberry PI 3 Model B} allows for 6,175 potential classifiers to be used in our moving target defense. In Figure~\ref{fig:hpcvsclass1}, different total HPCs have been log scaled graphed to show that an increase in the number of total HPCs available exponentially increases the number of potential classifiers that can be generated. Figure~\ref{fig:hpcvsclass1} shows that as the number of total HPCs increases, the growth appears to be exponential. Logically, this is reasonable because as the number of total HPCs increases, the number of different machine learning classifiers that can be generated will increase non-linearly. 


Now it is possible to see how many different total combinations of classifiers that are possible to have using N classifiers. Using the same total HPCs values from the first graph in figure~\ref{fig:hpcvsclass1}, the total number of classifiers were calculated through equation~\ref{equ6}, and then they were run through equation~\ref{equ9} to find the total number of combinations.
Figure~\ref{fig:hpcvscombo} is the log scaled graphed representation of equation \ref{equ9}. Results show that the graph is growing exponentially because an increase in N will result in a non-linear increase in the total number of combinations available. 

Visually, it can be seen that there are many different combinations of potential machine learning classifiers that can be utilized in the moving target defense. From the graphs, the smallest total HPC value we used was 20. This generated 6,715 possible classifiers as shown in equation~\ref{equ10}. When feeding that output into equation~\ref{equ9}, the result was approximately $7.248\times10^{1858}$. This is an enormous number that will only get even bigger as the total HPCs are increased. This provides really good defense from attackers trying to reverse engineer the moving target classifiers used because the attackers will not know which HPCs the classifiers are using, so they will have to test each combination. Out of $7.248\times10^{1858}$ total combinations for the {\it Raspberry PI 3 Model B}, only one of them is correct. The probability of guessing the right combination of classifiers used in the moving target defense is 1/ $7.248\times10^{1858}$ which is approximately $0.0000137969\times10^{-1858}$


\begin{figure}
  \includegraphics[width=\linewidth]{Figures/hpcvscombo.png}
  \caption{Log Scaled Number of Possible Combos based on Variation of Total HPCs}
  \label{fig:hpcvscombo}
\end{figure}

\end{comment}
